Efficient sequential Monte Carlo algorithms for integrated population models

State-space models are commonly used to describe different forms of ecological data. We consider the case of count data with observation errors. For such data the system process is typically multi-dimensional consisting of coupled Markov processes, where each component corresponds to a different characterisation of the population, such as age group, gender or breeding status. The associated system process equations describe the biological mechanisms under which the system evolves over time. However, there is often limited information in the count data alone to sensibly estimate demographic parameters of interest, so these are often combined with additional ecological observations leading to an integrated data analysis. Unfortunately, fitting these models to the data can be challenging, especially if the state-space model for the count data is non-linear or non-Gaussian. We propose an efficient particle Markov chain Monte Carlo algorithm to estimate the demographic parameters without the need for resorting to linear or Gaussian approximations. In particular, we exploit the integrated model structure to enhance the efficiency of the algorithm. We then incorporate the algorithm into a sequential Monte Carlo sampler in order to perform model comparison with regards to the dependence structure of the demographic parameters. Finally, we demonstrate the applicability and computational efficiency of our algorithms on two real datasets.

==> tracklang.tex <==
%%
%% This is file `tracklang.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tracklang.dtx  (with options: `tracklang.tex,package')
%% 
%%  tracklang.dtx
%%  Copyright 2015 Nicola Talbot
%% 
%%  This work may be distributed and/or modified under the
%%  conditions of the LaTeX Project Public License, either version 1.3
%%  of this license of (at your option) any later version.
%%  The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%%  and version 1.3 or later is part of all distributions of LaTeX
%%  version 2005/12/01 or later.
%% 
%%  This work has the LPPL maintenance status `maintained'.
%% 
%%  The Current Maintainer of this work is Nicola Talbot.
%% 
%%  This work consists of the files tracklang.dtx and tracklang.ins and the derived files tracklang.sty, tracklang.tex.
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
\ifx \@tracklang@languages\undefined
\else
  \expandafter\endinput
\fi
\long\def\@tracklang@ifundef#1#2#3{%
  \expandafter\ifx\csname #1\endcsname\relax
     #2%
  \else
     #3%
  \fi
}
\ifx\@nnil\undefined
  \def\@tracklang@nnil{\@nil}
\else
  \let\@tracklang@nnil\@nnil
\fi
\ifx\@for\undefined
  \long\def\@tracklang@for#1:=#2\do#3{%
    \expandafter\def\expandafter\@fortmp\expandafter{#2}%
    \ifx\@fortmp\empty
    \else
      \expandafter
        \@tracklang@forloop #2,\@nil,\@nil\@@ #1{#3}%
    \fi
  }
  \long\def\@tracklang@forloop#1,#2,#3\@@ #4#5{%
   \def #4{#1}%
   \ifx#4\@tracklang@nnil
   \else
     #5%
     \def #4{#2}%
     \ifx#4\@tracklang@nnil
     \else
       #5%
       \@tracklang@iforloop #3\@@ #4{#5}%
     \fi
   \fi
  }
  \long\def\@tracklang@iforloop#1,#2\@@ #3#4{%
    \def#3{#1}%
    \ifx#3\@tracklang@nnil
      \expandafter
        \@tracklang@fornoop
    \else
      #4\relax
      \expandafter\@tracklang@iforloop
    \fi
    #2\@@ #3{#4}%
  }
  \long\def\@tracklang@fornoop#1\@@ #2#3{}
\else
  \let\@tracklang@for\@for
\fi
\ifx\@namedef\undefined
  \def\@tracklang@namedef#1{\expandafter\def\csname#1\endcsname}
\else
  \let\@tracklang@namedef\@namedef
\fi
\ifx\@nameuse\undefined
  \def\@tracklang@nameuse#1{\csname#1\endcsname}
\else
  \let\@tracklang@nameuse\@nameuse
\fi
\ifx\PackageError\undefined
  \def\@tracklang@err#1#2{%
    \errehelp{#2}%
    \errmessage{tracklang: #1}}
\else
  \def\@tracklang@err#1#2{\PackageError{tracklang}{#1}{#2}}
\fi
\ifx\IfFileExists\undefined
 \long\def\@tracklang@IfFileExists#1#2#3{%
   \openin0=#1 %
   \ifeof0\relax
     \def\reserved@a{#3}%
   \else
     \closein0\relax
     \edef\@filef@und{#1 }%
     \def\reserved@a{#2}%
   \fi
   \reserved@a
 }

\else
  \let\@tracklang@IfFileExists\IfFileExists
\fi
\def\@tracklang@languages{}
\def\@tracklang@dialects{}
\def\@tracklang@ifinlist#1#2#3#4{%
  \def\@tracklang@doifinlist##1,#1,##2\end@tracklang@doifinlist{%
     \def\@before{##1}%
     \def\@after{##2}%
  }%
  \expandafter\@tracklang@doifinlist\expandafter,#2,#1,\@nil
    \end@tracklang@doifinlist
  \ifx\@after\@tracklang@nnil
    #4%
  \else
    #3%
  \fi
}
\def\@tracklang@add#1#2{%
  \edef\@tracklang@element{#1}%
  \ifx\@tracklang@element\empty
  \else
    \expandafter\@tracklang@ifinlist\expandafter{\@tracklang@element}#2%
    {%
    }%
    {%
     \ifx\empty#2\relax
       \let#2\@tracklang@element
     \else
       \edef#2{#2,\@tracklang@element}%
     \fi
    }%
  \fi
}
\def\AddTrackedDialect#1#2{%
 \@tracklang@add{#1}{\@tracklang@dialects}%
 \@tracklang@add{#2}{\@tracklang@languages}%
 \@tracklang@namedef{@tracklang@fromdialect@#1}{#2}%
 \@tracklang@ifundef{@tracklang@todialect@#2}%
 {\@tracklang@namedef{@tracklang@todialect@#2}{#1}}%
 {%
   \def\@tracklang@lang{#1}%
   \expandafter\@tracklang@add\expandafter\@tracklang@lang
     \csname @tracklang@todialect@#2\endcsname
 }%
}
\def\AddTrackedLanguage#1{%
  \AddTrackedDialect{#1}{#1}%
}
\def\AddTrackedIsoLanguage#1#2#3{%
  \@tracklang@namedef{@tracklang@#1@isofromlang@#3}{#2}%
  \@tracklang@ifundef{@tracklang@#1@isotolang@#2}%
  {\@tracklang@namedef{@tracklang@#1@isotolang@#2}{#3}}%
  {%
    \def\@tracklang@lang{#3}%
    \expandafter\@tracklang@add\expandafter\@tracklang@lang
      \csname @tracklang@#1@isotolang@#2\endcsname
  }%
}
\def\TrackedLanguageFromIsoCode#1#2{%
  \@tracklang@nameuse{@tracklang@#1@isotolang@#2}%
}
\def\TrackedIsoCodeFromLanguage#1#2{%
  \@tracklang@nameuse{@tracklang@#1@isofromlang@#2}%
}
\def\TrackedLanguageFromDialect#1{%
 \@tracklang@nameuse{@tracklang@fromdialect@#1}%
}
\def\TrackedDialectsFromLanguage#1{%
 \@tracklang@nameuse{@tracklang@todialect@#1}%
}
\def\TwoLetterIsoCountryCode{3166-1}
\def\TwoLetterIsoLanguageCode{639-1}
\def\ThreeLetterIsoLanguageCode{639-2}
\def\TrackPredefinedDialect#1{%
  \@tracklang@ifundef{@tracklang@add@#1}%
  {%
    \@tracklang@err{Dialect `#1' is not predefined}{}%
  }%
  {\@tracklang@nameuse{@tracklang@add@#1}}%
}
\ifx\@tracklang@declareoption\undefined
  \def\@tracklang@declareoption#1{}
\fi
\def\@tracklang@add@acadian{%
  \AddTrackedDialect{acadian}{french}%
  \AddTrackedIsoLanguage{639-1}{fr}{french}%
}
\@tracklang@declareoption{acadian}
\def\@tracklang@add@afrikaans{%
  \AddTrackedLanguage{afrikaans}%
  \AddTrackedIsoLanguage{639-1}{af}{afrikaans}%
  \AddTrackedIsoLanguage{639-2}{afr}{afrikaans}%
}
\@tracklang@declareoption{afrikaans}
\def\@tracklang@add@albanian{%
  \AddTrackedLanguage{albanian}%
  \AddTrackedIsoLanguage{639-1}{sq}{albanian}%
  \AddTrackedIsoLanguage{639-2-B}{alb}{albanian}%
  \AddTrackedIsoLanguage{639-2-T}{sqi}{albanian}%
  \AddTrackedIsoLanguage{639-2}{sqi}{albanian}%
}
\@tracklang@declareoption{albanian}
\def\@tracklang@add@amharic{%
  \AddTrackedLanguage{amharic}%
  \AddTrackedIsoLanguage{639-1}{am}{amharic}%
  \AddTrackedIsoLanguage{639-2}{amh}{amharic}%
}
\@tracklang@declareoption{amharic}
\def\@tracklang@add@anglosaxon{%
  \AddTrackedLanguage{anglosaxon}%
  \AddTrackedIsoLanguage{639-2}{ang}{anglosaxon}%
}
\@tracklang@declareoption{anglosaxon}
\def\@tracklang@add@apache{%
  \AddTrackedLanguage{apache}%
  \AddTrackedIsoLanguage{639-2}{apa}{apache}%
}
\@tracklang@declareoption{apache}
\def\@tracklang@add@arabic{%
  \AddTrackedLanguage{arabic}%
  \AddTrackedIsoLanguage{639-1}{ar}{arabic}%
  \AddTrackedIsoLanguage{639-2}{ara}{arabic}%
}
\@tracklang@declareoption{arabic}
\def\@tracklang@add@armenian{%
  \AddTrackedLanguage{armenian}%
  \AddTrackedIsoLanguage{639-1}{hy}{armenian}%
  \AddTrackedIsoLanguage{639-2-B}{arm}{armenian}%
  \AddTrackedIsoLanguage{639-2-T}{hye}{armenian}%
  \AddTrackedIsoLanguage{639-2}{hye}{armenian}%
}
\@tracklang@declareoption{armenian}
\def\@tracklang@add@asturian{%
  \AddTrackedLanguage{asturian}%
  \AddTrackedIsoLanguage{639-2}{ast}{asturian}%
}
\@tracklang@declareoption{asturian}
\def\@tracklang@add@american{%
  \AddTrackedDialect{american}{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
  \AddTrackedIsoLanguage{3166-1}{US}{american}%
}
\@tracklang@declareoption{american}
\def\@tracklang@add@australian{%
  \AddTrackedDialect{australian}{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
  \AddTrackedIsoLanguage{3166-1}{AU}{australian}%
}
\@tracklang@declareoption{australian}
\def\@tracklang@add@austrian{%
  \AddTrackedDialect{austrian}{german}%
  \AddTrackedIsoLanguage{639-1}{de}{german}%
  \AddTrackedIsoLanguage{639-2-B}{ger}{german}%
  \AddTrackedIsoLanguage{639-2-T}{deu}{german}%
  \AddTrackedIsoLanguage{639-2}{deu}{german}%
  \AddTrackedIsoLanguage{3166-1}{AT}{austrian}%
}
\@tracklang@declareoption{austrian}
\def\@tracklang@add@naustrian{%
  \AddTrackedDialect{naustrian}{german}%
  \AddTrackedIsoLanguage{639-1}{de}{german}%
  \AddTrackedIsoLanguage{639-2-B}{ger}{german}%
  \AddTrackedIsoLanguage{639-2-T}{deu}{german}%
  \AddTrackedIsoLanguage{639-2}{deu}{german}%
  \AddTrackedIsoLanguage{3166-1}{AT}{naustrian}%
}
\@tracklang@declareoption{naustrian}
\def\@tracklang@add@bahasa{%
  \AddTrackedDialect{bahasa}{bahasai}%
  \AddTrackedIsoLanguage{639-1}{id}{bahasai}%
  \AddTrackedIsoLanguage{639-2}{ind}{bahasai}%
  \AddTrackedIsoLanguage{3166-1}{IN}{bahasa}%
}
\@tracklang@declareoption{bahasa}
\def\@tracklang@add@bahasai{%
  \AddTrackedDialect{bahasai}{bahasai}%
  \AddTrackedIsoLanguage{639-1}{id}{bahasai}%
  \AddTrackedIsoLanguage{639-2}{ind}{bahasai}%
  \AddTrackedIsoLanguage{3166-1}{IN}{bahasai}%
}
\@tracklang@declareoption{bahasai}
\def\@tracklang@add@bahasam{%
  \AddTrackedLanguage{bahasam}%
  \AddTrackedIsoLanguage{639-1}{ms}{bahasam}%
  \AddTrackedIsoLanguage{639-2-B}{may}{bahasam}%
  \AddTrackedIsoLanguage{639-2-T}{msa}{bahasam}%
  \AddTrackedIsoLanguage{639-2}{msa}{bahasam}%
  \AddTrackedIsoLanguage{3166-1}{MY}{bahasam}%
}
\@tracklang@declareoption{bahasam}
\def\@tracklang@add@basque{%
  \AddTrackedLanguage{basque}%
  \AddTrackedIsoLanguage{639-1}{eu}{basque}%
  \AddTrackedIsoLanguage{639-2-B}{baq}{basque}%
  \AddTrackedIsoLanguage{639-2-T}{eus}{basque}%
  \AddTrackedIsoLanguage{639-2}{eus}{basque}%
}
\@tracklang@declareoption{basque}
\def\@tracklang@add@bengali{%
  \AddTrackedLanguage{bengali}%
  \AddTrackedIsoLanguage{639-1}{bn}{bengali}%
  \AddTrackedIsoLanguage{639-2}{ben}{bengali}%
}
\@tracklang@declareoption{bengali}
\def\@tracklang@add@brazil{%
  \AddTrackedDialect{brazil}{portuges}%
  \AddTrackedIsoLanguage{639-1}{pt}{portuges}%
  \AddTrackedIsoLanguage{639-2}{por}{portuges}%
  \AddTrackedIsoLanguage{3166-1}{BR}{brazil}%
}
\@tracklang@declareoption{brazil}
\def\@tracklang@add@brazilian{%
  \AddTrackedDialect{brazilian}{portuges}%
  \AddTrackedIsoLanguage{639-1}{pt}{portuges}%
  \AddTrackedIsoLanguage{639-2}{por}{portuges}%
  \AddTrackedIsoLanguage{3166-1}{BR}{brazilian}%
}
\@tracklang@declareoption{brazilian}
\def\@tracklang@add@breton{%
  \AddTrackedLanguage{breton}%
  \AddTrackedIsoLanguage{639-1}{br}{breton}%
  \AddTrackedIsoLanguage{639-2}{bre}{breton}%
  \AddTrackedIsoLanguage{3166-1}{FR}{breton}%
}
\@tracklang@declareoption{breton}
\def\@tracklang@add@british{%
  \AddTrackedDialect{british}{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
  \AddTrackedIsoLanguage{3166-1}{GB}{british}%
}
\@tracklang@declareoption{british}
\def\@tracklang@add@bulgarian{%
  \AddTrackedLanguage{bulgarian}%
  \AddTrackedIsoLanguage{639-1}{bg}{bulgarian}%
  \AddTrackedIsoLanguage{639-2}{bul}{bulgarian}%
}
\@tracklang@declareoption{bulgarian}
\def\@tracklang@add@canadian{%
  \AddTrackedDialect{canadian}{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
  \AddTrackedIsoLanguage{3166-1}{CA}{canadian}%
}
\@tracklang@declareoption{canadian}
\def\@tracklang@add@canadien{%
  \AddTrackedDialect{canadien}{french}%
  \AddTrackedIsoLanguage{639-1}{fr}{french}%
  \AddTrackedIsoLanguage{639-2-B}{fre}{french}%
  \AddTrackedIsoLanguage{639-2-T}{fra}{french}%
  \AddTrackedIsoLanguage{639-2}{fra}{french}%
  \AddTrackedIsoLanguage{3166-1}{CA}{canadien}%
}
\@tracklang@declareoption{canadien}
\def\@tracklang@add@catalan{%
  \AddTrackedLanguage{catalan}%
  \AddTrackedIsoLanguage{639-1}{ca}{catalan}%
  \AddTrackedIsoLanguage{639-2}{cat}{catalan}%
}
\@tracklang@declareoption{catalan}
\def\@tracklang@add@coptic{%
  \AddTrackedLanguage{coptic}%
  \AddTrackedIsoLanguage{639-2}{cop}{coptic}%
}
\@tracklang@declareoption{coptic}
\def\@tracklang@add@croatian{%
  \AddTrackedLanguage{croatian}%
  \AddTrackedIsoLanguage{639-1}{hr}{croatian}%
  \AddTrackedIsoLanguage{639-2}{hrv}{croatian}%
}
\@tracklang@declareoption{croatian}
\def\@tracklang@add@croatia{%
  \AddTrackedDialect{croatia}{croatian}%
  \AddTrackedIsoLanguage{639-1}{hr}{croatian}%
  \AddTrackedIsoLanguage{639-2}{hrv}{croatian}%
  \AddTrackedIsoLanguage{3166-1}{HR}{croatia}%
}
\@tracklang@declareoption{croatia}
\def\@tracklang@add@istriacountycroatian{%
  \AddTrackedDialect{istriacountycroatian}{croatian}%
  \AddTrackedIsoLanguage{639-1}{hr}{croatian}%
  \AddTrackedIsoLanguage{639-2}{hrv}{croatian}%
  \AddTrackedIsoLanguage{3166-1}{HR}{istriacountycroatian}%
}
\@tracklang@declareoption{istriacountycroatian}
\def\@tracklang@add@istriacountyitalian{%
  \AddTrackedDialect{istriacountyitalian}{italian}%
  \AddTrackedIsoLanguage{639-1}{it}{italian}%
  \AddTrackedIsoLanguage{639-2}{ita}{italian}%
  \AddTrackedIsoLanguage{3166-1}{HR}{istriacountyitalian}%
}
\@tracklang@declareoption{istriacountyitalian}
\def\@tracklang@add@czech{%
  \AddTrackedLanguage{czech}%
  \AddTrackedIsoLanguage{639-1}{cs}{czech}%
  \AddTrackedIsoLanguage{639-2-B}{cze}{czech}%
  \AddTrackedIsoLanguage{639-2-T}{ces}{czech}%
  \AddTrackedIsoLanguage{639-2}{ces}{czech}%
}
\@tracklang@declareoption{czech}
\def\@tracklang@add@danish{%
  \AddTrackedLanguage{danish}%
  \AddTrackedIsoLanguage{639-1}{da}{danish}%
  \AddTrackedIsoLanguage{639-2}{dan}{danish}%
}
\@tracklang@declareoption{danish}
\def\@tracklang@add@divehi{%
  \AddTrackedLanguage{divehi}%
  \AddTrackedIsoLanguage{639-1}{dv}{divehi}%
  \AddTrackedIsoLanguage{639-2}{div}{divehi}%
}
\@tracklang@declareoption{divehi}
\def\@tracklang@add@dutch{%
  \AddTrackedLanguage{dutch}%
  \AddTrackedIsoLanguage{639-1}{nl}{dutch}%
  \AddTrackedIsoLanguage{639-2-B}{dut}{dutch}%
  \AddTrackedIsoLanguage{639-2-T}{nld}{dutch}%
  \AddTrackedIsoLanguage{639-2}{nld}{dutch}%
}
\@tracklang@declareoption{dutch}
\def\@tracklang@add@netherlands{%
  \AddTrackedDialect{netherlands}{dutch}%
  \AddTrackedIsoLanguage{639-1}{nl}{dutch}%
  \AddTrackedIsoLanguage{639-2-B}{dut}{dutch}%
  \AddTrackedIsoLanguage{639-2-T}{nld}{dutch}%
  \AddTrackedIsoLanguage{639-2}{nld}{dutch}%
  \AddTrackedIsoLanguage{3166-1}{NL}{netherlands}%
}
\@tracklang@declareoption{netherlands}
\def\@tracklang@add@english{%
  \AddTrackedLanguage{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
}
\@tracklang@declareoption{english}
\def\@tracklang@add@esperanto{%
  \AddTrackedLanguage{esperanto}%
  \AddTrackedIsoLanguage{639-1}{eo}{esperanto}%
  \AddTrackedIsoLanguage{639-2}{epo}{esperanto}%
}
\@tracklang@declareoption{esperanto}
\def\@tracklang@add@estonian{%
  \AddTrackedLanguage{estonian}%
  \AddTrackedIsoLanguage{639-1}{et}{estonian}%
  \AddTrackedIsoLanguage{639-2}{est}{estonian}%
}
\@tracklang@declareoption{estonian}
\def\@tracklang@add@farsi{%
  \AddTrackedLanguage{farsi}%
  \AddTrackedIsoLanguage{639-1}{fa}{farsi}%
  \AddTrackedIsoLanguage{639-2-B}{per}{farsi}%
  \AddTrackedIsoLanguage{639-2-T}{fas}{farsi}%
  \AddTrackedIsoLanguage{639-2}{fas}{farsi}%
}
\@tracklang@declareoption{farsi}
\def\@tracklang@add@persian{%
  \AddTrackedDialect{persian}{farsi}%
  \AddTrackedIsoLanguage{639-1}{fa}{farsi}%
  \AddTrackedIsoLanguage{639-2-B}{per}{farsi}%
  \AddTrackedIsoLanguage{639-2-T}{fas}{farsi}%
  \AddTrackedIsoLanguage{639-2}{fas}{farsi}%
}
\@tracklang@declareoption{persian}
\def\@tracklang@add@finnish{%
  \AddTrackedLanguage{finnish}%
  \AddTrackedIsoLanguage{639-1}{fi}{finnish}%
  \AddTrackedIsoLanguage{639-2}{fin}{finnish}%
}
\@tracklang@declareoption{finnish}
\def\@tracklang@add@flemish{%
  \AddTrackedDialect{flemish}{dutch}%
  \AddTrackedIsoLanguage{639-1}{nl}{dutch}%
  \AddTrackedIsoLanguage{639-2-B}{dut}{dutch}%
  \AddTrackedIsoLanguage{639-2-T}{nld}{dutch}%
  \AddTrackedIsoLanguage{639-2}{nld}{dutch}%
  \AddTrackedIsoLanguage{3166-1}{BE}{flemish}%
}
\@tracklang@declareoption{flemish}
\def\@tracklang@add@francais{%
  \AddTrackedDialect{francais}{french}%
  \AddTrackedIsoLanguage{639-1}{fr}{french}%
  \AddTrackedIsoLanguage{639-2-B}{fre}{french}%
  \AddTrackedIsoLanguage{639-2-T}{fra}{french}%
  \AddTrackedIsoLanguage{639-2}{fra}{french}%
}
\@tracklang@declareoption{francais}
\def\@tracklang@add@frenchb{%
  \AddTrackedDialect{frenchb}{french}%
  \AddTrackedIsoLanguage{639-1}{fr}{french}%
  \AddTrackedIsoLanguage{639-2-B}{fre}{french}%
  \AddTrackedIsoLanguage{639-2-T}{fra}{french}%
  \AddTrackedIsoLanguage{639-2}{fra}{french}%
}
\@tracklang@declareoption{frenchb}
\def\@tracklang@add@french{%
  \AddTrackedLanguage{french}%
  \AddTrackedIsoLanguage{639-1}{fr}{french}%
  \AddTrackedIsoLanguage{639-2-B}{fre}{french}%
  \AddTrackedIsoLanguage{639-2-T}{fra}{french}%
  \AddTrackedIsoLanguage{639-2}{fra}{french}%
}
\@tracklang@declareoption{french}
\def\@tracklang@add@france{%
  \AddTrackedDialect{france}{french}%
  \AddTrackedIsoLanguage{639-1}{fr}{french}%
  \AddTrackedIsoLanguage{639-2-B}{fre}{french}%
  \AddTrackedIsoLanguage{639-2-T}{fra}{french}%
  \AddTrackedIsoLanguage{639-2}{fra}{french}%
  \AddTrackedIsoLanguage{3166-1}{FR}{france}%
}
\@tracklang@declareoption{france}
\def\@tracklang@add@belgique{%
  \AddTrackedDialect{belgique}{french}%
  \AddTrackedIsoLanguage{639-1}{fr}{french}%
  \AddTrackedIsoLanguage{639-2-B}{fre}{french}%
  \AddTrackedIsoLanguage{639-2-T}{fra}{french}%
  \AddTrackedIsoLanguage{639-2}{fra}{french}%
  \AddTrackedIsoLanguage{3166-1}{BE}{belgique}%
}
\@tracklang@declareoption{belgique}
\def\@tracklang@add@belgiangerman{%
  \AddTrackedDialect{belgiangerman}{german}%
  \AddTrackedIsoLanguage{639-1}{de}{german}%
  \AddTrackedIsoLanguage{639-2-B}{ger}{german}%
  \AddTrackedIsoLanguage{639-2-T}{deu}{german}%
  \AddTrackedIsoLanguage{639-2}{deu}{german}%
  \AddTrackedIsoLanguage{3166-1}{BE}{belgiangerman}%
}
\@tracklang@declareoption{belgiangerman}
\def\@tracklang@add@friulan{%
  \AddTrackedLanguage{friulan}%
  \AddTrackedIsoLanguage{639-2}{fur}{friulan}%
  \AddTrackedIsoLanguage{3166-1}{IT}{friulan}%
}
\@tracklang@declareoption{friulan}
\def\@tracklang@add@friulian{%
  \AddTrackedDialect{friulian}{friulan}%
  \AddTrackedIsoLanguage{639-2}{fur}{friulan}%
  \AddTrackedIsoLanguage{3166-1}{IT}{friulan}%
}
\@tracklang@declareoption{friulian}
\def\@tracklang@add@friulano{%
  \AddTrackedDialect{friulano}{friulan}%
  \AddTrackedIsoLanguage{639-2}{fur}{friulan}%
  \AddTrackedIsoLanguage{3166-1}{IT}{friulan}%
}
\@tracklang@declareoption{friulano}
\def\@tracklang@add@galician{%
  \AddTrackedLanguage{galician}%
  \AddTrackedIsoLanguage{639-1}{gl}{galician}%
  \AddTrackedIsoLanguage{639-2}{glg}{galician}%
}
\@tracklang@declareoption{galician}
\def\@tracklang@add@galicien{%
  \AddTrackedDialect{galicien}{galician}%
  \AddTrackedIsoLanguage{639-1}{gl}{galician}%
  \AddTrackedIsoLanguage{639-2}{glg}{galician}%
}
\@tracklang@declareoption{galicien}
\def\@tracklang@add@german{%
  \AddTrackedLanguage{german}%
  \AddTrackedIsoLanguage{639-1}{de}{german}%
  \AddTrackedIsoLanguage{639-2-B}{ger}{german}%
  \AddTrackedIsoLanguage{639-2-T}{deu}{german}%
  \AddTrackedIsoLanguage{639-2}{deu}{german}%
}
\@tracklang@declareoption{german}
\def\@tracklang@add@deutsch{%
  \AddTrackedDialect{deutsch}{german}%
  \AddTrackedIsoLanguage{639-1}{de}{german}%
  \AddTrackedIsoLanguage{639-2-B}{ger}{german}%
  \AddTrackedIsoLanguage{639-2-T}{deu}{german}%
  \AddTrackedIsoLanguage{639-2}{deu}{german}%
}
\@tracklang@declareoption{deutsch}
\def\@tracklang@add@ngerman{%
  \AddTrackedDialect{ngerman}{german}%
  \AddTrackedIsoLanguage{639-1}{de}{german}%
  \AddTrackedIsoLanguage{639-2-B}{ger}{german}%
  \AddTrackedIsoLanguage{639-2-T}{deu}{german}%
  \AddTrackedIsoLanguage{639-2}{deu}{german}%
}
\@tracklang@declareoption{ngerman}
\def\@tracklang@add@ngermanDE{%
  \AddTrackedDialect{ngerman}{german}%
  \AddTrackedIsoLanguage{639-1}{de}{german}%
  \AddTrackedIsoLanguage{639-2-B}{ger}{german}%
  \AddTrackedIsoLanguage{639-2-T}{deu}{german}%
  \AddTrackedIsoLanguage{639-2}{deu}{german}%
  \AddTrackedIsoLanguage{3166-1}{DE}{germany}%
}
\@tracklang@declareoption{ngermanDE}
\def\@tracklang@add@greek{%
  \AddTrackedLanguage{greek}%
  \AddTrackedIsoLanguage{639-1}{el}{greek}%
  \AddTrackedIsoLanguage{639-2-B}{gre}{greek}%
  \AddTrackedIsoLanguage{639-2-T}{ell}{greek}%
  \AddTrackedIsoLanguage{639-2}{ell}{greek}%
}
\@tracklang@declareoption{greek}
\def\@tracklang@add@hebrew{%
  \AddTrackedLanguage{hebrew}%
  \AddTrackedIsoLanguage{639-1}{he}{hebrew}%
  \AddTrackedIsoLanguage{639-2}{heb}{hebrew}%
}
\@tracklang@declareoption{hebrew}
\def\@tracklang@add@hindi{%
  \AddTrackedLanguage{hindi}%
  \AddTrackedIsoLanguage{639-1}{hi}{hindi}%
  \AddTrackedIsoLanguage{639-2}{hin}{hindi}%
}
\@tracklang@declareoption{hindi}
\def\@tracklang@add@hungarian{%
  \AddTrackedDialect{hungarian}{magyar}%
  \AddTrackedIsoLanguage{639-1}{hu}{magyar}%
  \AddTrackedIsoLanguage{639-2}{hun}{magyar}%
  \AddTrackedIsoLanguage{3166-1}{HU}{hungarian}%
}
\@tracklang@declareoption{hungarian}
\def\@tracklang@add@magyar{%
  \AddTrackedLanguage{magyar}%
  \AddTrackedIsoLanguage{639-1}{hu}{magyar}%
  \AddTrackedIsoLanguage{639-2}{hun}{magyar}%
}
\@tracklang@declareoption{magyar}
\def\@tracklang@add@icelandic{%
  \AddTrackedLanguage{icelandic}%
  \AddTrackedIsoLanguage{639-1}{is}{icelandic}%
  \AddTrackedIsoLanguage{639-2-B}{ice}{icelandic}%
  \AddTrackedIsoLanguage{639-2-T}{isl}{icelandic}%
  \AddTrackedIsoLanguage{639-2}{isl}{icelandic}%
}
\@tracklang@declareoption{icelandic}
\def\@tracklang@add@indon{%
  \AddTrackedDialect{indon}{bahasai}%
  \AddTrackedIsoLanguage{639-1}{id}{bahasai}%
  \AddTrackedIsoLanguage{639-2}{ind}{bahasai}%
  \AddTrackedIsoLanguage{3166-1}{IN}{indon}%
}
\@tracklang@declareoption{indon}
\def\@tracklang@add@indonesian{%
  \AddTrackedDialect{indonesian}{bahasai}%
  \AddTrackedIsoLanguage{639-1}{id}{bahasai}%
  \AddTrackedIsoLanguage{639-2}{ind}{bahasai}%
  \AddTrackedIsoLanguage{3166-1}{IN}{indonesian}%
}
\@tracklang@declareoption{indonesian}
\def\@tracklang@add@interlingua{%
  \AddTrackedLanguage{interlingua}%
  \AddTrackedIsoLanguage{639-1}{ia}{interlingua}%
  \AddTrackedIsoLanguage{639-2}{ina}{interlingua}%
}
\@tracklang@declareoption{interlingua}
\def\@tracklang@add@irish{%
  \AddTrackedLanguage{irish}%
  \AddTrackedIsoLanguage{639-1}{ga}{irish}%
  \AddTrackedIsoLanguage{639-2}{gle}{irish}%
}
\@tracklang@declareoption{irish}
\def\@tracklang@add@gaeilge{%
  \AddTrackedDialect{gaeilge}{irish}%
  \AddTrackedIsoLanguage{639-1}{ga}{irish}%
  \AddTrackedIsoLanguage{639-2}{gle}{irish}%
}
\@tracklang@declareoption{gaeilge}
\def\@tracklang@add@IEirish{%
  \AddTrackedDialect{IEirish}{irish}%
  \AddTrackedIsoLanguage{639-1}{ga}{irish}%
  \AddTrackedIsoLanguage{639-2}{gle}{irish}%
  \AddTrackedIsoLanguage{3166-1}{IE}{IEirish}%
}
\@tracklang@declareoption{IEirish}
\def\@tracklang@add@GBirish{%
  \AddTrackedDialect{GBirish}{irish}%
  \AddTrackedIsoLanguage{639-1}{ga}{irish}%
  \AddTrackedIsoLanguage{639-2}{gle}{irish}%
  \AddTrackedIsoLanguage{3166-1}{GB}{GBirish}%
}
\@tracklang@declareoption{GBirish}
\@tracklang@declareoption{IEenglish}
\def\@tracklang@add@IEenglish{%
  \AddTrackedDialect{IEenglish}{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
  \AddTrackedIsoLanguage{3166-1}{IE}{IEenglish}%
}
\@tracklang@declareoption{IEenglish}
\def\@tracklang@add@italian{%
  \AddTrackedLanguage{italian}%
  \AddTrackedIsoLanguage{639-1}{it}{italian}%
  \AddTrackedIsoLanguage{639-2}{ita}{italian}%
}
\@tracklang@declareoption{italian}
\def\@tracklang@add@italy{%
  \AddTrackedDialect{italy}{italian}%
  \AddTrackedIsoLanguage{639-1}{it}{italian}%
  \AddTrackedIsoLanguage{639-2}{ita}{italian}%
  \AddTrackedIsoLanguage{3166-1}{IT}{italy}%
}
\@tracklang@declareoption{italy}
\def\@tracklang@add@vatican{%
  \AddTrackedDialect{vatican}{italian}%
  \AddTrackedIsoLanguage{639-1}{it}{italian}%
  \AddTrackedIsoLanguage{639-2}{ita}{italian}%
  \AddTrackedIsoLanguage{3166-1}{VA}{vatican}%
}
\@tracklang@declareoption{vatican}
\def\@tracklang@add@sanmarino{%
  \AddTrackedDialect{sanmarino}{italian}%
  \AddTrackedIsoLanguage{639-1}{it}{italian}%
  \AddTrackedIsoLanguage{639-2}{ita}{italian}%
  \AddTrackedIsoLanguage{3166-1}{SM}{sanmarino}%
}
\@tracklang@declareoption{sanmarino}
\def\@tracklang@add@sloveneistriaitalian{%
  \AddTrackedDialect{sloveneistriaitalian}{italian}%
  \AddTrackedIsoLanguage{639-1}{it}{italian}%
  \AddTrackedIsoLanguage{639-2}{ita}{italian}%
  \AddTrackedIsoLanguage{3166-1}{SI}{sloveneistriaitalian}%
}
\@tracklang@declareoption{sloveneistriaitalian}
\def\@tracklang@add@jerseyenglish{%
  \AddTrackedDialect{jerseyenglish}{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
  \AddTrackedIsoLanguage{3166-1}{JE}{jerseyenglish}%
}
\@tracklang@declareoption{jerseyenglish}
\def\@tracklang@add@jerseyfrench{%
  \AddTrackedDialect{jerseyfrench}{french}%
  \AddTrackedIsoLanguage{639-1}{fr}{french}%
  \AddTrackedIsoLanguage{639-2-B}{fre}{french}%
  \AddTrackedIsoLanguage{639-2-T}{fra}{french}%
  \AddTrackedIsoLanguage{639-2}{fra}{french}%
  \AddTrackedIsoLanguage{3166-1}{JE}{jerseyfrench}%
}
\@tracklang@declareoption{jerseyfrench}
\def\@tracklang@add@guernseyenglish{%
  \AddTrackedDialect{guernseyenglish}{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
  \AddTrackedIsoLanguage{3166-1}{GG}{guernseyenglish}%
}
\@tracklang@declareoption{guernseyenglish}
\def\@tracklang@add@guernseyfrench{%
  \AddTrackedDialect{guernseyfrench}{french}%
  \AddTrackedIsoLanguage{639-1}{fr}{french}%
  \AddTrackedIsoLanguage{639-2-B}{fre}{french}%
  \AddTrackedIsoLanguage{639-2-T}{fra}{french}%
  \AddTrackedIsoLanguage{639-2}{fra}{french}%
  \AddTrackedIsoLanguage{3166-1}{GG}{guernseyfrench}%
}
\@tracklang@declareoption{guernseyfrench}
\def\@tracklang@add@kannada{%
  \AddTrackedLanguage{kannada}%
  \AddTrackedIsoLanguage{639-1}{kn}{kannada}%
  \AddTrackedIsoLanguage{639-2}{kan}{kannada}%
}
\@tracklang@declareoption{kannada}
\def\@tracklang@add@lao{%
  \AddTrackedLanguage{lao}%
  \AddTrackedIsoLanguage{639-1}{lo}{lao}%
  \AddTrackedIsoLanguage{639-2}{lao}{lao}%
}
\@tracklang@declareoption{lao}
\def\@tracklang@add@latin{%
  \AddTrackedLanguage{latin}%
  \AddTrackedIsoLanguage{639-1}{la}{latin}%
  \AddTrackedIsoLanguage{639-2}{lat}{latin}%
}
\@tracklang@declareoption{latin}
\def\@tracklang@add@latein{%
  \AddTrackedDialect{latein}{latin}%
  \AddTrackedIsoLanguage{639-1}{la}{latin}%
  \AddTrackedIsoLanguage{639-2}{lat}{latin}%
}
\@tracklang@declareoption{latein}
\def\@tracklang@add@latvian{%
  \AddTrackedLanguage{latvian}%
  \AddTrackedIsoLanguage{639-1}{lv}{latvian}%
  \AddTrackedIsoLanguage{639-2}{lav}{latvian}%
}
\@tracklang@declareoption{latvian}
\def\@tracklang@add@lithuanian{%
  \AddTrackedLanguage{lithuanian}%
  \AddTrackedIsoLanguage{639-1}{lt}{lithuanian}%
  \AddTrackedIsoLanguage{639-2}{lit}{lithuanian}%
}
\@tracklang@declareoption{lithuanian}
\def\@tracklang@add@lsorbian{%
  \AddTrackedLanguage{lsorbian}%
  \AddTrackedIsoLanguage{639-2}{dsb}{lsorbian}%
  \AddTrackedIsoLanguage{3166-1}{DE}{lsorbian}%
}
\@tracklang@declareoption{lsorbian}
\def\@tracklang@add@lowersorbian{%
  \AddTrackedDialect{lowersorbian}{lsorbian}%
  \AddTrackedIsoLanguage{639-2}{dsb}{lsorbian}%
  \AddTrackedIsoLanguage{3166-1}{DE}{lowersorbian}%
}
\@tracklang@declareoption{lowersorbian}
\def\@tracklang@add@malay{%
  \AddTrackedDialect{malay}{bahasam}%
  \AddTrackedIsoLanguage{639-1}{ms}{bahasam}%
  \AddTrackedIsoLanguage{639-2-B}{may}{bahasam}%
  \AddTrackedIsoLanguage{639-2-T}{msa}{bahasam}%
  \AddTrackedIsoLanguage{639-2}{msa}{bahasam}%
  \AddTrackedIsoLanguage{3166-1}{MY}{malay}%
}
\@tracklang@declareoption{malay}
\def\@tracklang@add@meyalu{%
  \AddTrackedDialect{meyalu}{bahasam}%
  \AddTrackedIsoLanguage{639-1}{ms}{bahasam}%
  \AddTrackedIsoLanguage{639-2-B}{may}{bahasam}%
  \AddTrackedIsoLanguage{639-2-T}{msa}{bahasam}%
  \AddTrackedIsoLanguage{639-2}{msa}{bahasam}%
  \AddTrackedIsoLanguage{3166-1}{MY}{meyalu}%
}
\@tracklang@declareoption{meyalu}
\def\@tracklang@add@maltese{%
  \AddTrackedLanguage{maltese}%
  \AddTrackedIsoLanguage{639-1}{mt}{maltese}%
  \AddTrackedIsoLanguage{639-2}{mlt}{maltese}%
}
\@tracklang@declareoption{maltese}
\def\@tracklang@add@maltamaltese{%
  \AddTrackedDialect{maltamaltese}{maltese}%
  \AddTrackedIsoLanguage{639-1}{mt}{maltese}%
  \AddTrackedIsoLanguage{639-2}{mlt}{maltese}%
  \AddTrackedIsoLanguage{3166-1}{MT}{maltamaltese}%
}
\@tracklang@declareoption{maltamaltese}
\def\@tracklang@add@maltaenglish{%
  \AddTrackedDialect{maltaenglish}{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
  \AddTrackedIsoLanguage{3166-1}{MT}{maltaenglish}%
}
\@tracklang@declareoption{maltaenglish}
\def\@tracklang@add@malayalam{%
  \AddTrackedLanguage{malayalam}%
  \AddTrackedIsoLanguage{639-1}{ml}{malayalam}%
  \AddTrackedIsoLanguage{639-2}{mal}{malayalam}%
}
\@tracklang@declareoption{malayalam}
\def\@tracklang@add@marathi{%
  \AddTrackedLanguage{marathi}%
  \AddTrackedIsoLanguage{639-1}{mr}{marathi}%
  \AddTrackedIsoLanguage{639-2}{mar}{marathi}%
}
\@tracklang@declareoption{marathi}
\def\@tracklang@add@newzealand{%
  \AddTrackedDialect{newzealand}{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
  \AddTrackedIsoLanguage{3166-1}{NZ}{newzealand}%
}
\@tracklang@declareoption{newzealand}
\def\@tracklang@add@isleofmanenglish{%
  \AddTrackedDialect{isleofmanenglish}{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
  \AddTrackedIsoLanguage{3166-1}{IM}{isleofmanenglish}%
}
\@tracklang@declareoption{isleofmanenglish}
\def\@tracklang@add@manx{%
  \AddTrackedLanguage{manx}%
  \AddTrackedIsoLanguage{639-1}{gv}{manx}%
  \AddTrackedIsoLanguage{639-2}{glv}{manx}%
  \AddTrackedIsoLanguage{3166-1}{IM}{manx}%
}
\@tracklang@declareoption{manx}
\def\@tracklang@add@nko{%
  \AddTrackedLanguage{nko}%
  \AddTrackedIsoLanguage{639-2}{nqo}{nko}%
}
\@tracklang@declareoption{nko}
\def\@tracklang@add@nynorsk{%
  \AddTrackedDialect{nynorsk}{norsk}%
  \AddTrackedIsoLanguage{639-1}{nn}{norsk}%
  \AddTrackedIsoLanguage{639-2}{nno}{norsk}%
  \AddTrackedIsoLanguage{3166-1}{NO}{nynorsk}%
}
\@tracklang@declareoption{nynorsk}
\def\@tracklang@add@norwegian{%
  \AddTrackedDialect{norwegian}{norsk}%
  \AddTrackedIsoLanguage{639-1}{nn}{norsk}%
  \AddTrackedIsoLanguage{639-2}{nno}{norsk}%
  \AddTrackedIsoLanguage{3166-1}{NO}{norwegian}%
}
\@tracklang@declareoption{norwegian}
\def\@tracklang@add@norsk{%
  \AddTrackedLanguage{norsk}%
  \AddTrackedIsoLanguage{639-1}{nn}{norsk}%
  \AddTrackedIsoLanguage{639-2}{nno}{norsk}%
  \AddTrackedIsoLanguage{3166-1}{NO}{norsk}%
}
\@tracklang@declareoption{norsk}
\def\@tracklang@add@occitan{%
  \AddTrackedLanguage{occitan}%
  \AddTrackedIsoLanguage{639-1}{oc}{occitan}%
  \AddTrackedIsoLanguage{639-2}{oci}{occitan}%
}
\@tracklang@declareoption{occitan}
\def\@tracklang@add@piedmontese{%
  \AddTrackedLanguage{piedmontese}%
  \AddTrackedIsoLanguage{3166-1}{IT}{piedmontese}%
}
\@tracklang@declareoption{piedmontese}
\def\@tracklang@add@piemonteis{%
  \AddTrackedDialect{piemonteis}{piedmontese}%
  \AddTrackedIsoLanguage{3166-1}{IT}{piemonteis}%
}
\@tracklang@declareoption{piemonteis}
\def\@tracklang@add@polish{%
  \AddTrackedLanguage{polish}%
  \AddTrackedIsoLanguage{639-1}{pl}{polish}%
  \AddTrackedIsoLanguage{639-2}{pol}{polish}%
}
\@tracklang@declareoption{polish}
\def\@tracklang@add@polutonikogreek{%
  \AddTrackedDialect{polutonikogreek}{greek}%
  \AddTrackedIsoLanguage{639-1}{el}{greek}%
  \AddTrackedIsoLanguage{639-2-B}{gre}{greek}%
  \AddTrackedIsoLanguage{639-2-T}{ell}{greek}%
  \AddTrackedIsoLanguage{639-2}{ell}{greek}%
}
\@tracklang@declareoption{polutonikogreek}
\def\@tracklang@add@polutoniko{%
  \AddTrackedDialect{polutoniko}{greek}%
  \AddTrackedIsoLanguage{639-1}{el}{greek}%
  \AddTrackedIsoLanguage{639-2-B}{gre}{greek}%
  \AddTrackedIsoLanguage{639-2-T}{ell}{greek}%
  \AddTrackedIsoLanguage{639-2}{ell}{greek}%
}
\@tracklang@declareoption{polutoniko}
\def\@tracklang@add@portuguese{%
  \AddTrackedDialect{portuguese}{portuges}%
  \AddTrackedIsoLanguage{639-1}{pt}{portuges}%
  \AddTrackedIsoLanguage{639-2}{por}{portuges}%
}
\@tracklang@declareoption{portuguese}
\def\@tracklang@add@portuges{%
  \AddTrackedLanguage{portuges}%
  \AddTrackedIsoLanguage{639-1}{pt}{portuges}%
  \AddTrackedIsoLanguage{639-2}{por}{portuges}%
}
\@tracklang@declareoption{portuges}
\def\@tracklang@add@portugal{%
  \AddTrackedDialect{portgual}{portuges}%
  \AddTrackedIsoLanguage{639-1}{pt}{portuges}%
  \AddTrackedIsoLanguage{639-2}{por}{portuges}%
  \AddTrackedIsoLanguage{3166-1}{PT}{portugal}%
}
\@tracklang@declareoption{portugal}
\def\@tracklang@add@romanian{%
  \AddTrackedLanguage{romanian}%
  \AddTrackedIsoLanguage{639-1}{ro}{romanian}%
  \AddTrackedIsoLanguage{639-2-B}{rum}{romanian}%
  \AddTrackedIsoLanguage{639-2-T}{ron}{romanian}%
  \AddTrackedIsoLanguage{639-2}{ron}{romanian}%
}
\@tracklang@declareoption{romanian}
\def\@tracklang@add@romansh{%
  \AddTrackedLanguage{romansh}%
  \AddTrackedIsoLanguage{639-1}{rm}{romansh}%
  \AddTrackedIsoLanguage{639-2}{roh}{romansh}%
}
\@tracklang@declareoption{romansh}
\def\@tracklang@add@romansch{%
  \AddTrackedDialect{romansch}{romansh}%
  \AddTrackedIsoLanguage{639-1}{rm}{romansh}%
  \AddTrackedIsoLanguage{639-2}{roh}{romansh}%
}
\@tracklang@declareoption{romansch}
\def\@tracklang@add@rumantsch{%
  \AddTrackedDialect{rumantsch}{romansh}%
  \AddTrackedIsoLanguage{639-1}{rm}{romansh}%
  \AddTrackedIsoLanguage{639-2}{roh}{romansh}%
}
\@tracklang@declareoption{rumantsch}
\def\@tracklang@add@romanche{%
  \AddTrackedDialect{romanche}{romansh}%
  \AddTrackedIsoLanguage{639-1}{rm}{romansh}%
  \AddTrackedIsoLanguage{639-2}{roh}{romansh}%
}
\@tracklang@declareoption{romanche}
\def\@tracklang@add@russian{%
  \AddTrackedLanguage{russian}%
  \AddTrackedIsoLanguage{639-1}{ru}{russian}%
  \AddTrackedIsoLanguage{639-2}{rus}{russian}%
}
\@tracklang@declareoption{russian}
\def\@tracklang@add@russianb{%
  \AddTrackedDialect{russianb}{russian}%
  \AddTrackedIsoLanguage{639-1}{ru}{russian}%
  \AddTrackedIsoLanguage{639-2}{rus}{russian}%
}
\@tracklang@declareoption{russianb}
\def\@tracklang@add@samin{%
  \AddTrackedLanguage{samin}%
  \AddTrackedIsoLanguage{639-1}{se}{samin}%
  \AddTrackedIsoLanguage{639-2}{sme}{samin}%
}
\@tracklang@declareoption{samin}
\def\@tracklang@add@sanskrit{%
  \AddTrackedLanguage{sanskrit}%
  \AddTrackedIsoLanguage{639-1}{sa}{sanskrit}%
  \AddTrackedIsoLanguage{639-2}{san}{sanskrit}%
}
\@tracklang@declareoption{sanskrit}
\def\@tracklang@add@scottish{%
  \AddTrackedLanguage{scottish}%
  \AddTrackedIsoLanguage{639-1}{gd}{scottish}%
  \AddTrackedIsoLanguage{639-2}{gla}{scottish}%
}
\@tracklang@declareoption{scottish}
\def\@tracklang@add@gaelic{%
  \AddTrackedDialect{gaelic}{scottish}%
  \AddTrackedIsoLanguage{639-1}{gd}{scottish}%
  \AddTrackedIsoLanguage{639-2}{gla}{scottish}%
}
\@tracklang@declareoption{gaelic}
\def\@tracklang@add@serbian{%
  \AddTrackedLanguage{serbian}%
  \AddTrackedIsoLanguage{639-1}{sr}{serbian}%
  \AddTrackedIsoLanguage{639-2}{srp}{serbian}%
}
\@tracklang@declareoption{serbian}
\def\@tracklang@add@slovak{%
  \AddTrackedLanguage{slovak}%
  \AddTrackedIsoLanguage{639-1}{sk}{slovak}%
  \AddTrackedIsoLanguage{639-2-B}{slo}{slovak}%
  \AddTrackedIsoLanguage{639-2-T}{slk}{slovak}%
  \AddTrackedIsoLanguage{639-2}{slk}{slovak}%
}
\@tracklang@declareoption{slovak}
\def\@tracklang@add@slovene{%
  \AddTrackedLanguage{slovene}%
  \AddTrackedIsoLanguage{639-1}{sl}{slovene}%
  \AddTrackedIsoLanguage{639-2}{slv}{slovene}%
}
\@tracklang@declareoption{slovene}
\def\@tracklang@add@slovenian{%
  \AddTrackedDialect{slovenian}{slovene}%
  \AddTrackedIsoLanguage{639-1}{sl}{slovene}%
  \AddTrackedIsoLanguage{639-2}{slv}{slovene}%
}
\@tracklang@declareoption{slovenian}
\def\@tracklang@add@slovenia{%
  \AddTrackedDialect{slovenia}{slovene}%
  \AddTrackedIsoLanguage{639-1}{sl}{slovene}%
  \AddTrackedIsoLanguage{639-2}{slv}{slovene}%
  \AddTrackedIsoLanguage{3166-1}{SI}{slovenia}%
}
\@tracklang@declareoption{slovenia}
\def\@tracklang@add@sloveneistriaslovenian{%
  \AddTrackedDialect{sloveneistriaslovenian}{slovenian}%
  \AddTrackedIsoLanguage{639-1}{sl}{slovene}%
  \AddTrackedIsoLanguage{639-2}{slv}{slovene}%
  \AddTrackedIsoLanguage{3166-1}{SI}{sloveneistriaslovenian}%
}
\@tracklang@declareoption{sloveneistriaslovenian}
\def\@tracklang@add@spanish{%
  \AddTrackedLanguage{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
}
\@tracklang@declareoption{spanish}
\def\@tracklang@add@spainspanish{%
  \AddTrackedDialect{spainspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{ES}{spainspanish}%
}
\@tracklang@declareoption{spainspanish}
\def\@tracklang@add@argentinespanish{%
  \AddTrackedDialect{argentinespanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{AR}{argentinespanish}%
}
\@tracklang@declareoption{argentinespanish}
\def\@tracklang@add@bolivianspanish{%
  \AddTrackedDialect{bolivianspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{BO}{bolivianspanish}%
}
\@tracklang@declareoption{bolivianspanish}
\def\@tracklang@add@chilianspanish{%
  \AddTrackedDialect{chilianspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{CL}{chilianspanish}%
}
\@tracklang@declareoption{chilianspanish}
\def\@tracklang@add@columbianspanish{%
  \AddTrackedDialect{columbianspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{CO}{columbianspanish}%
}
\@tracklang@declareoption{columbianspanish}
\def\@tracklang@add@costaricanspanish{%
  \AddTrackedDialect{costaricanspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{CR}{costaricanspanish}%
}
\@tracklang@declareoption{costaricanspanish}
\def\@tracklang@add@cubanspanish{%
  \AddTrackedDialect{cubanspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{CU}{cubanspanish}%
}
\@tracklang@declareoption{cubanspanish}
\def\@tracklang@add@dominicanspanish{%
  \AddTrackedDialect{dominicanspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{DO}{dominicanspanish}%
}
\@tracklang@declareoption{dominicanspanish}
\def\@tracklang@add@ecudorianspanish{%
  \AddTrackedDialect{ecudorianspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{EC}{ecudorianspanish}%
}
\@tracklang@declareoption{ecudorianspanish}
\def\@tracklang@add@elsalvadorspanish{%
  \AddTrackedDialect{elsalvadorspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{SV}{elsalvadorspanish}%
}
\@tracklang@declareoption{elsalvadorspanish}
\def\@tracklang@add@guatemalanspanish{%
  \AddTrackedDialect{guatemalanspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{GT}{guatemalanspanish}%
}
\@tracklang@declareoption{guatemalanspanish}
\def\@tracklang@add@honduranspanish{%
  \AddTrackedDialect{honduranspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{HN}{honduranspanish}%
}
\@tracklang@declareoption{honduranspanish}
\def\@tracklang@add@mexicanspanish{%
  \AddTrackedDialect{mexicanspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{MX}{mexicanspanish}%
}
\@tracklang@declareoption{mexicanspanish}
\def\@tracklang@add@nicaraguanspanish{%
  \AddTrackedDialect{nicaraguanspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{NI}{nicaraguanspanish}%
}
\@tracklang@declareoption{nicaraguanspanish}
\def\@tracklang@add@panamaspanish{%
  \AddTrackedDialect{panamaspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{PA}{panamaspanish}%
}
\@tracklang@declareoption{panamaspanish}
\def\@tracklang@add@paraguayspanish{%
  \AddTrackedDialect{paraguayspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{PY}{paraguayspanish}%
}
\@tracklang@declareoption{paraguayspanish}
\def\@tracklang@add@peruvianspanish{%
  \AddTrackedDialect{peruvianspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{PE}{peruvianspanish}%
}
\@tracklang@declareoption{peruvianspanish}
\def\@tracklang@add@puertoricospanish{%
  \AddTrackedDialect{puertoricospanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{PR}{puertoricospanish}%
}
\@tracklang@declareoption{puertoricospanish}
\def\@tracklang@add@uruguayspanish{%
  \AddTrackedDialect{uruguayspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{UY}{uruguayspanish}%
}
\@tracklang@declareoption{uruguayspanish}
\def\@tracklang@add@venezuelanspanish{%
  \AddTrackedDialect{venezuelanspanish}{spanish}%
  \AddTrackedIsoLanguage{639-1}{es}{spanish}%
  \AddTrackedIsoLanguage{639-2}{spa}{spanish}%
  \AddTrackedIsoLanguage{3166-1}{VE}{venezuelanspanish}%
}
\@tracklang@declareoption{venezuelanspanish}
\def\@tracklang@add@swedish{%
  \AddTrackedLanguage{swedish}%
  \AddTrackedIsoLanguage{639-1}{sv}{swedish}%
  \AddTrackedIsoLanguage{639-2}{swe}{swedish}%
}
\@tracklang@declareoption{swedish}
\def\@tracklang@add@swissgerman{%
  \AddTrackedDialect{swissgerman}{german}%
  \AddTrackedIsoLanguage{639-1}{de}{german}%
  \AddTrackedIsoLanguage{639-2-B}{ger}{german}%
  \AddTrackedIsoLanguage{639-2-T}{deu}{german}%
  \AddTrackedIsoLanguage{639-2}{deu}{german}%
  \AddTrackedIsoLanguage{3166-1}{CH}{swissgerman}%
}
\@tracklang@declareoption{swissgerman}
\def\@tracklang@add@swissfrench{%
  \AddTrackedDialect{swissfrench}{french}%
  \AddTrackedIsoLanguage{639-1}{fr}{french}%
  \AddTrackedIsoLanguage{639-2-B}{fre}{french}%
  \AddTrackedIsoLanguage{639-2-T}{fra}{french}%
  \AddTrackedIsoLanguage{639-2}{fra}{french}%
  \AddTrackedIsoLanguage{3166-1}{CH}{swissfrench}%
}
\@tracklang@declareoption{swissfrench}
\def\@tracklang@add@swissitalian{%
  \AddTrackedDialect{swissitalian}{italian}%
  \AddTrackedIsoLanguage{639-1}{it}{italian}%
  \AddTrackedIsoLanguage{639-2}{ita}{italian}%
  \AddTrackedIsoLanguage{3166-1}{CH}{swissitalian}%
}
\@tracklang@declareoption{swissitalian}
\def\@tracklang@add@swissromansh{%
  \AddTrackedDialect{swissromansh}{romansh}%
  \AddTrackedIsoLanguage{639-1}{rm}{romansh}%
  \AddTrackedIsoLanguage{639-2}{roh}{romansh}%
  \AddTrackedIsoLanguage{3166-1}{CH}{swissromansh}%
}
\@tracklang@declareoption{swissromansh}
\def\@tracklang@add@syriac{%
  \AddTrackedLanguage{syriac}%
  \AddTrackedIsoLanguage{639-2}{syr}{syriac}%
}
\@tracklang@declareoption{syriac}
\def\@tracklang@add@tamil{%
  \AddTrackedLanguage{tamil}%
  \AddTrackedIsoLanguage{639-1}{ta}{tamil}%
  \AddTrackedIsoLanguage{639-2}{tam}{tamil}%
}
\@tracklang@declareoption{tamil}
\def\@tracklang@add@telugu{%
  \AddTrackedLanguage{telugu}%
  \AddTrackedIsoLanguage{639-1}{te}{telugu}%
  \AddTrackedIsoLanguage{639-2}{tel}{telugu}%
}
\@tracklang@declareoption{telugu}
\def\@tracklang@add@tai{%
  \AddTrackedLanguage{tai}%
  \AddTrackedIsoLanguage{639-2}{tai}{tai}%
}
\@tracklang@declareoption{tai}
\def\@tracklang@add@thai{%
  \AddTrackedLanguage{thai}%
  \AddTrackedIsoLanguage{639-1}{th}{thai}%
  \AddTrackedIsoLanguage{639-2}{tha}{thai}%
}
\@tracklang@declareoption{thai}
\def\@tracklang@add@tibetan{%
  \AddTrackedLanguage{tibetan}%
  \AddTrackedIsoLanguage{639-1}{bo}{tibetan}%
  \AddTrackedIsoLanguage{639-2-B}{tib}{tibetan}%
  \AddTrackedIsoLanguage{639-2-T}{bod}{tibetan}%
  \AddTrackedIsoLanguage{639-2}{bod}{tibetan}%
}
\@tracklang@declareoption{tibetan}
\def\@tracklang@add@turkish{%
  \AddTrackedLanguage{turkish}%
  \AddTrackedIsoLanguage{639-1}{tr}{turkish}%
  \AddTrackedIsoLanguage{639-2}{tur}{turkish}%
}
\@tracklang@declareoption{turkish}
\def\@tracklang@add@turkmen{%
  \AddTrackedLanguage{turkmen}%
  \AddTrackedIsoLanguage{639-1}{tk}{turkmen}%
  \AddTrackedIsoLanguage{639-2}{tuk}{turkmen}%
}
\@tracklang@declareoption{turkmen}
\def\@tracklang@add@UKenglish{%
  \AddTrackedDialect{UKenglish}{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
  \AddTrackedIsoLanguage{3166-1}{GB}{UKenglish}%
}
\@tracklang@declareoption{UKenglish}
\def\@tracklang@add@ukrainian{%
  \AddTrackedLanguage{ukrainian}%
  \AddTrackedIsoLanguage{639-1}{uk}{ukrainian}%
  \AddTrackedIsoLanguage{639-2}{ukr}{ukrainian}%
  \AddTrackedIsoLanguage{3166-1}{UA}{ukrainian}%
}
\@tracklang@declareoption{ukrainian}
\def\@tracklang@add@ukraineb{%
  \AddTrackedDialect{ukraineb}{ukrainian}%
  \AddTrackedIsoLanguage{639-1}{uk}{ukrainian}%
  \AddTrackedIsoLanguage{639-2}{ukr}{ukrainian}%
  \AddTrackedIsoLanguage{3166-1}{UA}{ukraineb}%
}
\@tracklang@declareoption{ukraineb}
\def\@tracklang@add@ukraine{%
  \AddTrackedDialect{ukraine}{ukrainian}%
  \AddTrackedIsoLanguage{639-1}{uk}{ukrainian}%
  \AddTrackedIsoLanguage{639-2}{ukr}{ukrainian}%
  \AddTrackedIsoLanguage{3166-1}{UA}{ukraine}%
}
\@tracklang@declareoption{ukraine}
\def\@tracklang@add@urdu{%
  \AddTrackedLanguage{urdu}%
  \AddTrackedIsoLanguage{639-1}{ur}{urdu}%
  \AddTrackedIsoLanguage{639-2}{urd}{urdu}%
}
\@tracklang@declareoption{urdu}
\def\@tracklang@add@usorbian{%
  \AddTrackedLanguage{usorbian}%
  \AddTrackedIsoLanguage{639-2}{dsb}{usorbian}%
  \AddTrackedIsoLanguage{3166-1}{DE}{usorbian}%
}
\@tracklang@declareoption{usorbian}
\def\@tracklang@add@uppersorbian{%
  \AddTrackedDialect{uppersorbian}{usorbian}%
  \AddTrackedIsoLanguage{639-2}{hsb}{usorbian}%
  \AddTrackedIsoLanguage{3166-1}{DE}{uppersorbian}%
}
\@tracklang@declareoption{uppersorbian}
\def\@tracklang@add@USenglish{%
  \AddTrackedDialect{USenglish}{english}%
  \AddTrackedIsoLanguage{639-1}{en}{english}%
  \AddTrackedIsoLanguage{639-2}{eng}{english}%
  \AddTrackedIsoLanguage{3166-1}{US}{USenglish}%
}
\@tracklang@declareoption{USenglish}
\def\@tracklang@add@valencian{%
  \AddTrackedDialect{valencian}{catalan}%
  \AddTrackedIsoLanguage{639-1}{ca}{catalan}%
  \AddTrackedIsoLanguage{639-2}{cat}{catalan}%
}
\@tracklang@declareoption{valencian}
\def\@tracklang@add@valencien{%
  \AddTrackedDialect{valencien}{catalan}%
  \AddTrackedIsoLanguage{639-1}{ca}{catalan}%
  \AddTrackedIsoLanguage{639-2}{cat}{catalan}%
}
\@tracklang@declareoption{valencien}
\def\@tracklang@add@vietnamese{%
  \AddTrackedLanguage{vietnamese}%
  \AddTrackedIsoLanguage{639-1}{vi}{vietnamese}%
  \AddTrackedIsoLanguage{639-2}{vie}{vietnamese}%
}
\@tracklang@declareoption{vietnamese}
\def\@tracklang@add@walloon{%
  \AddTrackedLanguage{walloon}%
  \AddTrackedIsoLanguage{639-1}{wa}{walloon}%
  \AddTrackedIsoLanguage{639-2}{wln}{walloon}%
}
\@tracklang@declareoption{walloon}
\def\@tracklang@add@welsh{%
  \AddTrackedLanguage{welsh}%
  \AddTrackedIsoLanguage{639-1}{cy}{welsh}%
  \AddTrackedIsoLanguage{639-2-B}{wel}{welsh}%
  \AddTrackedIsoLanguage{639-2-T}{cym}{welsh}%
  \AddTrackedIsoLanguage{639-2}{cym}{welsh}%
}
\@tracklang@declareoption{welsh}
\def\@tracklang@add@cymraeg{%
  \AddTrackedDialect{cymraeg}{welsh}%
  \AddTrackedIsoLanguage{639-1}{cy}{welsh}%
  \AddTrackedIsoLanguage{639-2-B}{wel}{welsh}%
  \AddTrackedIsoLanguage{639-2-T}{cym}{welsh}%
  \AddTrackedIsoLanguage{639-2}{cym}{welsh}%
}
\@tracklang@declareoption{cymraeg}
\def\LetTrackLangOption#1#2{%
  \expandafter\let\csname @tracklang@add@#1\expandafter\endcsname
    \csname @tracklang@add@#2\endcsname
  \@tracklang@declareoption{#1}%
}
\LetTrackLangOption{en-US}{american}
\LetTrackLangOption{en-GB}{british}
\LetTrackLangOption{en-AU}{australian}
\LetTrackLangOption{en-NZ}{newzealand}
\LetTrackLangOption{en-CA}{canadian}
\LetTrackLangOption{fr-CA}{canadien}
\LetTrackLangOption{fr-BE}{belgique}
\LetTrackLangOption{pt-BR}{brazilian}
\LetTrackLangOption{it-HR}{istriacountyitalian}
\LetTrackLangOption{nl-BE}{flemish}
\LetTrackLangOption{fr-FR}{france}
\LetTrackLangOption{de-DE}{ngermanDE}
\LetTrackLangOption{de-BE}{belgiangerman}
\LetTrackLangOption{en-GG}{guernseyenglish}
\LetTrackLangOption{fr-GG}{guernseyfrench}
\LetTrackLangOption{it-IT}{italy}
\LetTrackLangOption{mt-MT}{maltamaltese}
\LetTrackLangOption{en-MT}{maltaenglish}
\LetTrackLangOption{en-IM}{isleofmanenglish}
\LetTrackLangOption{en-JE}{jerseyenglish}
\LetTrackLangOption{fr-JE}{jerseyfrench}
\LetTrackLangOption{nl-NL}{netherlands}
\LetTrackLangOption{pt-PT}{portugal}
\LetTrackLangOption{it-SM}{sanmarino}
\LetTrackLangOption{sl-SI}{slovenia}
\LetTrackLangOption{it-SI}{sloveneistriaitalian}
\LetTrackLangOption{es-ES}{spainspanish}
\LetTrackLangOption{es-AR}{argentinespanish}
\LetTrackLangOption{es-BO}{bolivianspanish}
\LetTrackLangOption{es-CL}{chilianspanish}
\LetTrackLangOption{es-CO}{columbianspanish}
\LetTrackLangOption{es-CR}{costaricanspanish}
\LetTrackLangOption{es-CU}{cubanspanish}
\LetTrackLangOption{es-DO}{dominicanspanish}
\LetTrackLangOption{es-EC}{ecudorianspanish}
\LetTrackLangOption{es-SV}{elsalvadorspanish}
\LetTrackLangOption{es-GT}{guatemalanspanish}
\LetTrackLangOption{es-HN}{honduranspanish}
\LetTrackLangOption{es-MX}{mexicanspanish}
\LetTrackLangOption{es-NI}{nicaraguanspanish}
\LetTrackLangOption{es-PA}{panamaspanish}
\LetTrackLangOption{es-PY}{paraguayspanish}
\LetTrackLangOption{es-PE}{peruvianspanish}
\LetTrackLangOption{es-PR}{puertoricospanish}
\LetTrackLangOption{es-UY}{uruguayspanish}
\LetTrackLangOption{es-VE}{venezuelanspanish}
\LetTrackLangOption{de-CH}{swissgerman}
\LetTrackLangOption{fr-CH}{swissfrench}
\LetTrackLangOption{it-CH}{swissitalian}
\LetTrackLangOption{rm-CH}{swissromansh}
\LetTrackLangOption{it-VA}{vatican}
\LetTrackLangOption{ga-IE}{IEirish}
\LetTrackLangOption{ga-GB}{GBirish}
\LetTrackLangOption{en-IE}{IEenglish}
\long\def\IfTrackedLanguage#1#2#3{%
  \edef\@tracklang@element{#1}%
  \ifx\@tracklang@element\empty
    #3%
  \else
    \expandafter\@tracklang@ifinlist\expandafter{\@tracklang@element}%
      \@tracklang@languages
    {%
      #2%
    }%
    {%
      #3%
    }%
  \fi
}
\long\def\IfTrackedDialect#1#2#3{%
  \@tracklang@ifundef{@tracklang@fromdialect@#1}{#3}{#2}%
}
\long\def\IfTrackedIsoCode#1#2#3#4{%
  \@tracklang@ifundef{@tracklang@#1@isotolang@#2}{#4}{#3}%
}
\long\def\IfTrackedLanguageHasIsoCode#1#2#3#4{%
  \@tracklang@ifundef{@tracklang@#1@isofromlang@#2}{#4}{#3}%
}
\long\def\ForEachTrackedLanguage#1#2{%
  \@tracklang@for#1:=\@tracklang@languages\do{#2}%
}
\long\def\ForEachTrackedDialect#1#2{%
  \@tracklang@for#1:=\@tracklang@dialects\do{#2}%
}
\long\def\AnyTrackedLanguages#1#2{%
  \ifx\@tracklang@languages\empty
    #2%
  \else
    #1%
  \fi
}
\long\def\IfTrackedLanguageFileExists#1#2#3#4#5{%
   \def\CurrentTrackedTag{}%
   \def\CurrentTrackedDialect{#1}%
   \def\CurrentTrackedLanguage{}%
   \def\CurrentTrackedRegion{}%
   \def\CurrentTrackedIsoCode{}%
   \IfTrackedDialect{#1}%
   {%
     \IfTrackedLanguageHasIsoCode{3166-1}{#1}%
     {%
       \edef\CurrentTrackedRegion{%
         \TrackedIsoCodeFromLanguage{3166-1}{#1}}%
     }%
     {}%
     \edef\CurrentTrackedLanguage{\TrackedLanguageFromDialect{#1}}%
     \edef\CurrentTrackedTag{#1}%
     \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
     {#4}%
     {%
       \IfTrackedLanguageHasIsoCode
         {639-1}{\CurrentTrackedLanguage}
       {%
          \edef\CurrentTrackedIsoCode{%
             \TrackedIsoCodeFromLanguage
               {639-1}{\CurrentTrackedLanguage}}%
          \ifx\CurrentTrackedRegion\@empty
            \let\CurrentTrackedTag\CurrentTrackedIsoCode
            \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
            {#4}
            {%
              \IfTrackedLanguageHasIsoCode
                {639-2}{\CurrentTrackedLanguage}
              {%
                 \edef\CurrentTrackedIsoCode{%
                    \TrackedIsoCodeFromLanguage
                      {639-2}{\CurrentTrackedLanguage}}%
                 \let\CurrentTrackedTag\CurrentTrackedIsoCode
                 \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                 {#4}%
                 {%
                   \let\CurrentTrackedTag\CurrentTrackedLanguage
                   \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
                 }%
              }%
              {%
               \let\CurrentTrackedTag\CurrentTrackedLanguage
               \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
              }%
            }%
          \else
            \edef\CurrentTrackedTag{%
              \CurrentTrackedIsoCode-\CurrentTrackedRegion}%
            \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
            {#4}
            {%
              \IfTrackedLanguageHasIsoCode
              {639-2}{\CurrentTrackedLanguage}
              {%
                \let\org@currenttrackedisocode\CurrentTrackedIsoCode
                \edef\CurrentTrackedIsoCode{%
                  \TrackedIsoCodeFromLanguage
                  {639-2}{\CurrentTrackedLanguage}}%
                \edef\CurrentTrackedTag{%
                  \CurrentTrackedIsoCode-\CurrentTrackedRegion}%
                \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                {#4}%
                {%
                  \let\CurrentTrackedTag\org@currenttrackedisocode
                  \let\org@currenttrackedisocode\CurrentTrackedIsoCode
                  \let\CurrentTrackedIsoCode\CurrentTrackedTag
                  \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                  {#4}
                  {%
                    \let\CurrentTrackedIsoCode\org@currenttrackedisocode
                    \let\CurrentTrackedTag\CurrentTrackedIsoCode
                    \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                    {#4}%
                    {%
                      \let\CurrentTrackedTag\CurrentTrackedRegion
                      \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                      {#4}%
                      {%
                        \let\CurrentTrackedTag\CurrentTrackedLanguage
                        \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
                      }%
                    }%
                  }%
                }%
              }%
              {%
                \let\CurrentTrackedTag\CurrentTrackedIsoCode
                \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                {#4}%
                {%
                  \let\CurrentTrackedTag\CurrentTrackedRegion
                  \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                  {#4}%
                  {%
                    \let\CurrentTrackedTag\CurrentTrackedLanguage
                    \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
                  }%
                }%
              }%
            }%
          \fi
       }%
       {%
         \IfTrackedLanguageHasIsoCode
           {639-2}{\CurrentTrackedLanguage}
         {%
            \edef\CurrentTrackedIsoCode{%
               \TrackedIsoCodeFromLanguage
               {639-2}{\CurrentTrackedLanguage}}%
            \ifx\CurrentTrackedRegion\@empty
              \let\CurrentTrackedTag\CurrentTrackedIsoCode
              \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
              {#4}%
              {%
                \let\CurrentTrackedTag\CurrentTrackedLanguage
                \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
              }%
            \else
              \edef\CurrentTrackedTag{%
                \CurrentTrackedIsoCode-\CurrentTrackedRegion}%
              \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
              {#4}%
              {%
                \let\CurrentTrackedTag\CurrentTrackedIsoCode
                \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                {#4}%
                {%
                  \let\CurrentTrackedTag\CurrentTrackedRegion
                  \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
                  {#4}%
                  {%
                    \let\CurrentTrackedTag\CurrentTrackedLanguage
                    \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
                  }%
                }%
              }%
            \fi
         }%
         {%
           \ifx\CurrentTrackedRegion\@empty
             \let\CurrentTrackedTag\CurrentTrackedLanguage
             \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
           \else
             \let\CurrentTrackedTag\CurrentTrackedRegion
             \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}%
             {#4}%
             {%
               \let\CurrentTrackedTag\CurrentTrackedLanguage
               \@tracklang@IfFileExists{#2\CurrentTrackedTag#3}{#4}{#5}%
             }%
           \fi
         }%
       }%
     }%
   }%
   {#5}% unknown dialect
}
\endinput
%%
%% End of file `tracklang.tex'.

